On information captured by neural networks: connections with memorization and generalization

Despite the popularity and success of deep learning, there is limited understanding of when, how, and why neural networks generalize to unseen examples. Since learning can be seen as extracting information from data, we formally study information captured by neural networks during training. Specifically, we start with viewing learning in presence of noisy labels from an information-theoretic perspective and derive a learning algorithm that limits label noise information in weights. We then define a notion of unique information that an individual sample provides to the training of a deep network, shedding some light on the behavior of neural networks on examples that are atypical, ambiguous, or belong to underrepresented subpopulations. We relate example informativeness to generalization by deriving nonvacuous generalization gap bounds. Finally, by studying knowledge distillation, we highlight the important role of data and label complexity in generalization. Overall, our findings contribute to a deeper understanding of the mechanisms underlying neural network generalization.

==> dedication.tex <==
To everyone.


==> unique-info/sections/linearized-nets.tex <==
Linearized neural networks are a class of neural networks that can be obtained by taking first-order Taylor expansion of standard neural networks at their initialization~\citep{lee2019wide}:
\begin{equation*}
f^\mathrm{lin}_w(x) \triangleq f_{w_0}(x) + \nabla_w f_w(x)^T|_{w=w_0} (w - w_0).
\end{equation*}
This networks are linear with respect to their parameters, but can be highly non-linear with respect to input $x$.
\todo{why are linearized nets good?}.
Continuous-time gradient descent dynamics of linearized neural networks is
\begin{equation*}
\dot w_t = -\eta \left(\nabla_{f_t^\mathrm{lin}(X)} \Loss\right)^T \nabla_w f_0(X),
\end{equation*}
where $\eta > 0$ is the learning rate.
One of the advantages of linearized neural networks over standard neural networks is that the solution of the differential equation above can be written analytically if the loss function is mean squared error (MSE):
\begin{equation}
w_t = \nabla_w f_0(X) \Theta_0^{-1} \left(I - e^{-\eta \Theta_0 t}\right) (f_0(X) - Y),
\label{eq:lin-weights-at-t}
\end{equation}
where $\Theta_0 = \nabla_w f_0(X)^T\nabla_w f_0(X) \in \mathbb{R}^{nk \times nk}$ is the neural tangent kernel (NTK)\citep{jacot2018ntk, lee2019wide}.
Note that the NTK matrix will generally be invertible for overparametrized neural networks, as we usually have $d \gg nk$.
Having \cref{eq:lin-weights-at-t}, we can write down equations for predictions as well:
\begin{equation}
f^\mathrm{lin}_t(x) = f_0(x) + \Theta_0(x, X) \Theta_0^{-1} \left(I - e^{-\eta \Theta_0 t}\right) (Y - f_0(X)),
\label{eq:lin-preds-at-t}
\end{equation}
where $\Theta_0(x,X) = \nabla_w f_0(x)^T\nabla_w f_0(X) \in \mathbb{R}^{k \times nk}$.
Analogs of \cref{eq:lin-weights-at-t,eq:lin-preds-at-t} for discrete-time gradient descent can also be derived and correspond to replacing $e^{-\eta t \Theta_0}$ with $(I - \eta \Theta_0)^t$.
When weight decay of from $\frac{\lambda}{2} \lVert w - w_0\rVert_2^2$ is added, the only change that happens to \cref{eq:lin-weights-at-t,eq:lin-preds-at-t} is that $\Theta_0$ gets replaced by $(\Theta_0 + \lambda I)$, as we show in the \cref{sec:wd-linearized} of appendix.

Finally, int the case of MSE loss, the Hessian of training loss $\Loss(w)$ is equal to 
\begin{equation}
    H = \nabla f_0(X) \nabla f_0(X)^T + \lambda I,
    \label{eq:linearized-hessian}
\end{equation}
and is invertible if $\lambda > 0$.
Hereafter, we will focus on linearized neural networks, so instead of using $f^\mathrm{lin}_w(x)$ notation, we will use the shorter $f_w(x)$ notation.

